FOX: Hardware-Assisted File Auditing for Direct Access NVM-Hosted Filesystems

With emerging non-volatile memories entering the mainstream market, several operating systems start to incorporate new changes and optimizations. One major OS support is the direct-access for files, which enables efficient access for files hosted in byte-addressable NVM systems. With DAX-enabled filesystems, files can be accessed directly similar to memory with typical load/store operations. Despite its efficiency, the frequently used system call of direct access is troublesome for system auditing. File system auditing is mandatory and widely used because auditing logs can help detect anomalies, suspicious file accesses, or be used as an evidence in digital forensics. However, the frequent and long-time usage of direct access call blinds the operating system or file system from tracking process operations to shared files after the initial page faults. This might results in imprecise casualty analysis and leads to false conclusion for attack detection. To remedy the tension between enabling fine-grained file system auditing and leveraging the performance of NVM-hosted file systems, we propose a novel hardware-assisted auditing scheme, FOX. FOX enables file system auditing through lightweight hardware-software changes which can monitor every read or write event for mapped files on NVM. Additionally, we propose the optimized schemes, that enable auditing flexibility for selected files/memory range. By prototyping FOX on a full system simulator, Gem5, we observe a relatively small reduced throughput and an acceptable extra writes compared to our baseline. Compared to other instrumentation-based software schemes, our scheme is low-overhead and secure.

==> abstract.tex <==
\section{Abstract}
Filesystem auditing has been widely used in sensitive systems, e.g., defense computing systems. Auditing is mainly used to trace (or detect) any potential anomalies, suspicious file accesses, or used as an evidence in digital forensics. While filesystem auditing is a major requirement in many systems, the shift towards emerging Non-Volatile Memories (NVMs) would compulsory disable filesystem auditing. The main reason behinds such incompatibility between filesystem auditing and emerging NVMs is that NVM-hosted filesystems will be accessed directly through regular load/store operations, and hence abstracting away much of the software functions including auditing. Unfortunately, this will lead to either deploy NVMs as block devices (not directly accessible) so the software layer observes each access, and hence auditing is enabled, or completely disable auditing.      

To remedy the tension between enabling filesystem auditing and direct-access in NVM-hosted filesystems, we propose a novel hardware-assisted auditing scheme (\textit{FOX}). FOX enables filesystem auditing through lightweight hardware-software changes which can essentially enable filesystem auditing when direct access NVM-hosted filesystems are used. Thus, FOX enables the performance potentials of emerging NVMs by allowing direct fine-granularity accesses (as regular load/store operations), however, also enables filesystem auditing. We also discuss the impact of FOX on write-endurance of NVMs, performance and possible optimizations. By prototyping FOX on a full-system simulator, Gem5, we observe an average performance overhead of only 9 to 6.4\% reduced throughput and 58.3\% reduced writes compared to our baseline. 
